Maintaining Contour Trees of Dynamic Terrains

We consider maintaining the contour tree $\mathbb{T}$ of a piecewise-linear triangulation $\mathbb{M}$ that is the graph of a time varying height function $h: \mathbb{R}^2 \rightarrow \mathbb{R}$. We carefully describe the combinatorial change in $\mathbb{T}$ that happen as $h$ varies over time and how these changes relate to topological changes in $\mathbb{M}$. We present a kinetic data structure that maintains the contour tree of $h$ over time. Our data structure maintains certificates that fail only when $h(v)=h(u)$ for two adjacent vertices $v$ and $u$ in $\mathbb{M}$, or when two saddle vertices lie on the same contour of $\mathbb{M}$. A certificate failure is handled in $O(\log(n))$ time. We also show how our data structure can be extended to handle a set of general update operations on $\mathbb{M}$ and how it can be applied to maintain topological persistence pairs of time varying functions.

==> topology.tex <==
\section{Continuous Height Change} \label{sec:deformation}
Our algorithm maintains the contour tree $\contourtree$ of $\terrain$ while
allowing the height of vertices in $\terrain$ to be changed. More formally, we
support the $\changeheight(v,r)$ operation, that given a vertex $v$ in
$\terrain$ changes the height of $v$ to $r$ while updating $\contourtree$ to
reflect any topological changes that might be caused by the height change.
Besides $\contourtree$, we also maintain a descent tree $\descendtree(x)$ for
every minimum $x$ and an ascent tree $\ascendtree(y)$ for every maximum $y$ of
$\terrain$. These are auxiliary structures augmented to $\contourtree$ such
that a minimum vertex $x$ in $\contourtree$ stores $\descendtree(x)$ and a
maximum vertex $y$ in $\contourtree$ stores $\ascendtree(y)$. 
% Refer to Figure~\ref{fig:subdivisions} (c).

We process a $\changeheight(v,r)$ operation as a continuous deformation of
$\terrain$ over time, that changes the height of $v$ to $r$. During this
continuous deformation the combinatorial structure of $\contourtree$ changes
only at discrete time instances, called \emph{events}. For simplicity, we
assume that no multiple saddle vertex is created during this deformation.

Edelsbrunner et al.~\cite{} showed that if $h$ is a smooth function, then the
topology of $\contourtree$ changes when (i) a critical point $u$ becomes
degenerate (i.e. the Hessian at $u$ becomes singular), or (ii)
$\height(u)=\height(v)$ for two saddle points $u$ and $v$ and both $u$ and $v$
lie on the same contour. In either case, one of the edges of $\contourtree$ is
degenerate in the sense that the interval $[h(u), h(v)]$ is a single point.
In our setting, where $h$ is a piecewise-linear function, (i)
corresponds to two adjacent vertices $u$ and $v$ with $\height(u)=\height(v)$
and one of them being a saddle and the other an extremal vertex; (ii)
corresponds to two saddle vertices lying on the same contour. The former is
called a \emph{birth} or a \emph{death} event and the latter is called an
\emph{interchange} event.

Besides these two events, there is another event in the piecewise-linear case,
namely, a critical point shifts from one vertex to its neighbor --- no new
critical points are created, none is destroyed, and the topology of
$\contourtree$ does not change. Only the label of a node in $\contourtree$
changes. We refer to this event as the \emph{shift} event.

Finally, the ascent and descent trees also change at certain time instances, when
an oriented edge $(u,v)$ will be replaced with another edge $(u,w)$ or with the
edge $(v, u)$.

The birth, death, shift, and auxiliary events will be referred to as \emph{local}
events because they only occur when the height of two adjacent vertices
becomes equal.

Before we describe the events in detail we introduce a few notation. During the
deformation, we use $\heighttime{t} : \mesh \rightarrow \mathbb{R}$ to denote the
height function at time $t$. Note that during $\changeheight(v, r)$,
$\heighttime{t}$ changes only for points in $\star(v)$. If an event occurs at time
$t$, then we refer to $t^-$ (resp. $t^+$) as the time $t-\varepsilon$ (resp.
$t+\varepsilon)$ for some arbitrarily small $\varepsilon > 0$.

\subsection{Local events}
Suppose a local event occurs at time $t_0$ at which
$\heighttime{t_0}(v) = \heighttime{t_0}(u)$ where $u$ is a neighbor of
$v$. For simplicity, we assume that $\heighttime{t_0^-}(v) <
\heighttime{t_0^-}(u)$ and $\heighttime{t_0^+}(v) >
\heighttime{t_0^+}(u)$, i.e., the height of $v$ is being raised.
The other case when $\heighttime{t_0^-}(v) >
\heighttime{t_0^-}(u)$ is symmetric, simply reverse the direction of time. In
the following sections we describe in detail the changes that occur to
$\contourtree$ during the three kinds of local events. We assume the interval
$[t_0^-,t_0^+]$ sufficiently small so that there is no vertex $w \neq u,v$
whose height lies between those of $u$ and $v$ during this interval.

\paragraph{Auxiliary event} An auxiliary event occurs at $t_0$ if $(v,u)$ is
an edge in an ascent tree or $(u,v)$ is an edge in a descent tree.

First, suppose $(v,u)$ is an edge of an ascent tree at $t_0^-$. We remove the
edge $(v,u)$. If $v$ becomes a maximum vertex at $t_0^+$, then $v$ becomes the
root of an ascent tree; otherwise, we choose another vertex $w$ from
$\upperlink(v)$ and add the edge $(v,w)$. If $u$ was a maximum at $t_0^-$, i.e.,
$u$ is the root of an ascent tree, then we add the edge $(u,v)$.

Next, suppose $(u,v)$ is an edge in a descent tree at $t_0^-$. We delete the edge
$(u,v)$. If $u$ becomes a minimum vertex at $t_0^+$, $u$ becomes the root of a
descent tree; otherwise we choose a vertex $w$ from $\lowerlink(u)$ and add the
edge $(u,w)$. If $v$ was a minimum vertex at $t_0^-$, it is no longer a minimum
at $t_0^+$ and we add the edge $(v,u)$.

\paragraph{Shift event} A shift event occurs at $t_0$ if one of $u$ and
$v$, say $v$, was a critical vertex and other vertex, $u$, was a regular vertex
at $t_0^-$, and the critical vertex shifts from $v$ to $u$ at $t_0^+$. This
event does not cause any change in the topology of $\contourtree$ but the node
of $\contourtree$ that was labeled $v$ changes its label to $u$. If
$\heighttime{t_0^+}(v) > \heighttime{t_0^-}(v)$, i.e., $v$ is being raised
then at time $t_0^+$, $\retract(v)$ lies on an edge of $\contourtree$ whose
lower endpoint is $u$.

\paragraph{Birth/death event} 
A \emph{birth event} occurs at time $t_0$ if both $u$ and $v$ were
regular vertices at $t_0^-$, and they become critical vertices at
$t_0^+$. A \emph{death event} occurs when both $u$ and $v$ were critical
vertices at $t_0^-$ and become regular vertices at $t_0^+$. See
Figure~\ref{fig:birthdeath} for the change in the topology of $\contourtree$.
We now describe in detail how $\contourtree$ changes at a birth or a death
event.

\begin{figure} 
\centering
\includegraphics[width=0.15\textwidth, page=7]{figures/local-event}
\caption{Illustration of the change in the topology of the contour tree in birth and death events}
\label{fig:birthdeath}
\end{figure}

\textit{\textbf{Birth event:}}
If $v$ is being raised, then there are two possibilities: (i) $v$ becomes a
negative saddle and $u$ a minimum, or (ii) $v$ becomes a maximum and
$u$ a positive saddle. Suppose $\retract(u), \retract(v)$ lie on the
edge $(\alpha, \beta)$ of $\contourtree$. Then we split $(\alpha,
\beta)$ into two edges by adding a node corresponding to the new
saddle and creating a new edge incident on this node whose other
endpoint is a leaf. In case (i), $v$ is the node added on $(\alpha,
\beta)$ and $u$ is a new leaf, and in (ii) $u$ is the node on the edge
$(\alpha, \beta)$ and $v$ is the new leaf. 

\textit{\textbf{Death event:}}
Again, if $v$ is being raised, then there are two possibilities: (i) $v$ is a
minimum and $u$ a negative saddle at $t_0^-$, and (ii) $v$ is a positive saddle
and $u$ a maximum at $t_0^-$. In either case the edge $(u,v)$ disappears from
$\contourtree$ at $t_0^+$. Two edges incident on this degree 2 vertex merge
into a single edge.

\paragraph{Proof of correctness}
We now prove that whenever a local event occurs, then either the topology of
$\contourtree$ changes because of a birth/death event or the label of a node in
$\contourtree$ changes because of a shift event. There are three cases
depending on whether $u$ is an extremal, saddle or a regular vertex at time
$t_0^-$.
\\\\
(i) \emph{$v$ is an extremal vertex at time $t_0^-$.}  
Since $\heighttime{h_0^-}(v) < \heighttime{h_0^-}(u)$, $v$ cannot be a maximum
at time $t_0^-$, so assume that $v$ is a minimum at $t_0^-$. We observe that
$u$ also cannot be a maximum vertex because for any $w \in \link(v) \cup
\link(u)$, $\heighttime{t_0^-}(w) > \heighttime{t_0^-}(v)$, and therefore
$\heighttime{t_0^-}(w) > \heighttime{t_0^-}(u)$.  If $u$ is a \emph{regular
vertex} at time $t_0^-$. Then $v$ is the only vertex in $\lowerlink(u)$ at
$t_0^-$. At time $t_0$ a shift event occurs that shifts the minimum from $v$ to
$u$. At $t_0^+$, $v$ is a regular vertex with $\lowerlink(v)=u$. 

If $u$ is a saddle vertex at time $t_0^-$, then at time $t_0$ a death event
occurs such that both $v$ and $u$ are regular vertices at time $t_0^+$. See
Figure~\ref{fig:local-event} (a) 
\\\\
(ii) \emph{$v$ is a regular vertex at time $t_0^-$.} 
If $u$ is the only vertex in $\upperlink(v)$, then $v$ becomes a maximum
vertex. If $u$ is a maximum at $t_0^-$, then a shift event occurs at $t_0$ and
$u$ becomes a regular vertex at $t_0^+$, and if $u$ is a regular vertex at
$t_0^-$ then a birth event occurs at $t_0$ and $u$ becomes a saddle vertex at
$t_0^+$; see Figure~\ref{fig:local-event} (b) (Note that $u$ cannot be a saddle
vertex at $t_0^-$ because otherwise $u$ becomes a multiple saddle at $t_0^+$.)

If $\upperlink(v)$ contains multiple vertices and $u$ is an endpoint of
$\upperlink(v)$ (degree of $u$ in $\upperlink(v)$ is 1), then $v$ simply
remains a regular vertex at $t_0^+$ and $u$ switches from $\upperlink(v)$ to
$\lowerlink(v)$. This does not cause $\contourtree$ to change. 

Finally, if $u$ is a middle vertex in $\upperlink(v)$ (degree of $w$ in
$\upperlink(v)$ is 2), $v$ becomes a saddle vertex at time $t_0^+$. If $u$ is
a regular vertex at time $t_0^-$, a birth event occurs at $t_0$ that creates a
minimum vertex at $u$ at $t_0^+$. If $u$ is a saddle vertex at time $t_0^-$,
then a shift event occurs at $t_0$ and becomes a regular vertex at $t_0^+$.
\\\\
(iii) \emph{$v$ is a saddle vertex at time}
$t_0^-$.  Note that since we assume that no multiple saddles can be created
during deformation, $u$ can not be the middle vertex of $\upperlink(v)$ at time
$t_0^-$.  If $u$ is the only vertex in $\upperlink(v)$, then $v$ becomes a
regular vertex. If $u$ is a regular vertex at $t_0^-$, then a shift event
occurs at $t_0$ and $u$ becomes a saddle vertex at $t_0^+$, and if $u$ is a
maximum vertex at $t_0^-$ then a death event occurs at $t_0$ and $u$ becomes a
regular vertex at $t_0^+$; see Figure~\ref{fig:local-event} (c).  (Note that $u$
cannot be a saddle vertex at $t_0^-$ because otherwise $u$  becomes a multiple
saddle at $t_0^+$.)

Finally, If $u$ is an endpoint of $\upperlink(v)$
neither $v$ nor $u$ changes vertex type. 

\begin{figure} 
\centering
\begin{tabular}{|>{\centering\arraybackslash}m{0.5cm}|>{\centering\arraybackslash}m{7cm}|>{\centering\arraybackslash}m{7cm}|}
\hline
& \emph{Shift event} & \emph{Birth / Death event} \\
\hline
\hline
(a)
& \includegraphics[width=0.42\textwidth, page=1]{figures/local-event} 
& \includegraphics[width=0.42\textwidth, page=2]{figures/local-event} \\
\hline
(b)
& \includegraphics[width=0.42\textwidth, page=3]{figures/local-event} 
& \includegraphics[width=0.42\textwidth, page=4]{figures/local-event} \\
\hline
(c)
& \includegraphics[width=0.42\textwidth, page=5]{figures/local-event} 
& \includegraphics[width=0.42\textwidth, page=6]{figures/local-event} \\
\hline
\end{tabular}
\caption{Illustration of local events. (a) is when $v$ is a minimum vertex. (b)
is when $v$ is a regular vertex. (c) is when $v$ is a saddle vertex}
\label{fig:local-event}
\end{figure}


\subsection{Interchange events}
An interchange event occurs at time $t_0$ if there are two saddle
vertices $\alpha, \beta$ such that $\heighttime{t_0}(\alpha) =
\heighttime{t_0}(\beta)$ and both $\alpha$ and $\beta$ lie on the same
contour, i.e., $\retract(\alpha) = \retract(\beta)$ at time $t_0$. There are
four cases depending on whether $\alpha$ and $\beta$ are positive or negative
saddles.  Suppose $\heighttime{t_0^-}(\alpha) < \heighttime{t_0^-}(\beta)$.
Without loss of generality assume that $\alpha$ is a negative saddle. The other
case, when $\alpha$ is positive can be reduced to this case by
reversing the $z$-axis and/or time axis; see below. Then there are two
cases: (i) both $\alpha$ and $\beta$ are negative saddles, and (ii)
$\alpha$ is negative and $\beta$ is positive. We refer to them
as \emph{negative} and \emph{mixed} interchange events.  We describe these
events and their effect on $\contourtree$ in detail in the following sections,
but first we introduce some notation. For any contour, we label its vertices
that lie on the edges incident on $\alpha$ (resp. $\beta$) with $\alpha$ (resp.
$\beta$). We also note that at time $t_0^-$ (or $t_0^+$) all contours in the
equivalence class ($\alpha$, $\beta$) are combinatorially identical because no
vertex of $\mesh$ retracts to the edge ($\alpha$, $\beta$) of $\contourtree$.
Let $\cycle_{\alpha = \beta}$ denote the contour at time $t_0$ passing through both
$\alpha$ and $\beta$. \jungwoo{The case where $\alpha$ and $\beta$ are neighbor
in $\mesh$ should be mentioned and it can be avoid because it is a monkey
saddle}

\subsubsection{Negative interchange event} \label{sec:neg-interchange}
Let $\ada, \adb$ be the two down neighbors of $\alpha$ at $t_0^-$, and let
$\bua$ be the other down neighbor of $\beta$ ($\alpha$ is a down neighbor
of $\beta$ at $t_0^-$). See Figure~\ref{fig:transitions}. The
change in topology of $\contourtree$ at a negative interchange event is similar
to performing a rotation at node $\beta$. That is, $\alpha$ becomes the upper
endpoint and $\beta$ the lower endpoint of the edge $(\alpha, \beta)$ at time
$t_0^+$, and one of the down subtrees of $\alpha$ (rooted in $\ada$ and $\adb$)
becomes a down subtree of $\beta$. Next we describe the change of
$\contourtree$ in more detail, and also argue why our analysis is correct.

% \begin{figure} 
% \centering
% \begin{tabular}{>{\centering}m{4cm}>{\centering}m{2cm}>{\centering}m{4cm}}
% \includegraphics[width=0.25\textwidth, page=1]{figures/negative-interchange-tree} 
% & $\longleftrightarrow$
% & \includegraphics[width=0.25\textwidth, page=2]{figures/negative-interchange-tree} \\
% \end{tabular}
% \caption{Illustration of contour tree in a negative interchange event}
% \label{fig:negative-interchange-tree}
% \end{figure}

% \paragraph{Contour tree changes}
Let $\cycle_\beta^-$ be the contour passing through $\beta$ at time $t_0^-$. It
consists of two simple polygonal cycles $\cycle_{\alpha\beta}^-$ and
$\cycle_{\bua\beta}^-$, belonging to the equivalence classes of contours
corresponding to the edges $(\alpha,\beta)$ and $(\bua, \beta)$ of
$\contourtree$, respectively; $\beta$ is the only common point of
$\cycle_{\alpha\beta}^-$ and $\cycle_{\bua\beta}^-$.  Similarly, let
$\cycle_{\alpha}^-$ denote the contour passing through $\alpha$ at $t_0^-$, and
let $\cycle_{\ada\alpha}^-, \cycle_{\adb\alpha}^-$ be its two simple cycles
connected at $\alpha$. 

Recall that all contours corresponding to the edge $(\alpha, \beta)$ are
combinatorially identical. For any such contour $\cycle^-$, the vertices marked
$\beta$ appear in one connected interval. Therefore only one of the two cycles
$\cycle_{\ada\alpha}^-, \cycle_{\adb\alpha}^-$ of $\cycle_\alpha^-$, say
$\cycle_{\adb\alpha}^-$, contains the vertices marked $\beta$.

\begin{lemma}
If $\cycle_{\adb\alpha}^-$ contains the vertices marked $\beta$, then at time
$t_0^+$, $\adb$ becomes a down neighbor of $\beta$, $\bua$ the other down neighbor of
$\beta$, and $\ada$ and $\beta$ becomes the down neighbor of $\alpha$.
\end{lemma}
\begin{proof}
Fix a height $\theta = \heighttime{t_0^-}(\alpha) - \delta$ for an arbitrary small
parameter $\delta > 0$. Let $\cycle_\ada^-, \cycle_\adb^-$, and $\cycle_\bua^-$ be the
contours at height $\theta$ at time $t_0^-$ corresponding to the edges $(\ada,
\alpha), (\adb,\alpha)$, and $(\bua, \beta)$, and let $\cycle_\ada^+,
\cycle_\adb^+, \cycle_\bua^+$ be the contours at height $\theta$ corresponding
to $\cycle_\ada^-, \cycle_\adb^-, \cycle_\bua^-$, respectively, at time
$t_0^+$. Note that $\cycle_\ada^-$, and $\cycle_\adb^-$ have vertices marked
$\alpha$; $\cycle_\adb^-$ and $\cycle_\bua^-$ have vertices marked $\beta$; and
$\seqedge(\cycle_\ada^-) = \seqedge(\cycle_\ada^+), \seqedge(\cycle_\adb^-) =
\seqedge(\cycle_\adb^+)$, and $\seqedge(\cycle_\bua^-) =
\seqedge(\cycle_\bua^+)$.

We now fix time at $t_0^+$. Recall that $\theta < \heighttime{t_0^+}(\beta) <
\heighttime{t_0^+}(\alpha)$. As we increase the height from $\theta$ to
$\heighttime{t_0^+}(\beta)$, the contours $\cycle_\ada^+, \cycle_\adb^+$, and
$\cycle_\bua^+$ continuously deform. The vertices marked $\beta$ in
$\cycle_\adb^+$ and $\cycle_\bua^+$ converge to $\beta$, and thus
$\cycle_\adb^+$ and $\cycle_\bua^+$ merge into a single contour at $\beta$.
Thus $\beta$ is a negative saddle and has $\adb$ and $\bua$ as its down neighbors.

Next, we increase the height from $\heighttime{t_0^+}(\beta)$ to $\heighttime{t_0^+}(\alpha)$.
The merged contour of $\cycle_\adb^+$ and $\cycle_\bua^+$, denoted by
$\cycle_{\beta\alpha}^+$, contains vertices marked $\alpha$ and so does the
contour $\cycle_\bua^+$. Hence as the height reaches $\alpha$, the vertices marked
$\alpha$ in $\cycle_{\beta\alpha}^+$ and $\cycle_\bua^+$ converge to $\alpha$. 
Hence at time $t_0^+$, $\alpha$ is a negative saddle with $\beta$ and $\bua$ as
its two down neighbors. This completes the proof of the lemma.
\end{proof}

Next, we analyze the change in colors of $\alpha$ and $\beta$ at the above
event. There are three cases depending on the colors of $\alpha$ and $\beta$ at
time $t_0^-$.

First, assume that $\beta$ is blue at $t_0^-$, then $\alpha$ is also blue at
$t_0^-$, and so are the cycles $\cycle_{\alpha\beta}^-, \cycle_{\bua\beta}^-,
\cycle_{\ada\alpha}^-, \cycle_{\adb\beta}^-$. See Figure~\ref{fig:transitions}
(a). Moreover, $\cycle_{\alpha\beta}^-, \cycle_{\bua\beta}^-$ lie in the exterior
of each other and so do $\cycle_{\ada\alpha}^-$ and $\cycle_{\adb\alpha}^-$.
Consequently $\cycle_\ada^-, \cycle_\adb^-, \cycle_\bua^-$ lie in the exterior
of each other, and the same holds for $\cycle_\ada^+, \cycle_\adb^+$, and
$\cycle_\bua^+$. We can now conclude that $\alpha$ and $\beta$ remain blue
negative saddles at time $t_0^+$.

Next, assume that $\beta$ is red at $t_0^-$. Then one of $(\alpha, \beta)$ or
$(\bua, \beta)$ is red and the other is blue. We assume that $(\alpha, \beta)$
is red; we will argue below that the other case can be reduced to this case. In
this case $\cycle_{\bua\beta}^-$ lies in the interior of the cycle
$\cycle_{\alpha\beta}^-$; see Figure~\ref{fig:transitions} (b), (c). If $\alpha$ is
red, then one of $(\ada,\alpha)$ and $(\adb, \alpha)$ is red and the other is
blue. First assume that $(\adb, \alpha)$ is red at $t_0^-$. So
$\cycle_{\ada\alpha}^-$ lies in the interior of $\cycle_{\adb\alpha}^-$: see
Figure~\ref{fig:transitions} (b). Hence $\cycle_{\adb}^-$ contains both
$\cycle_\ada^-$ and $\cycle_\bua^-$ in its interior. Therefore at time $t_0$,
the contour $\cycle_{\alpha=\beta}$ passing through $\alpha$ and $\beta$
consists of three cycles $\cycle_{\ada\alpha}, \cycle_{\adb\alpha}$, and
$\cycle_{\bua\beta}$ --- $\cycle_{\adb\alpha}$ containing both
$\cycle_{\ada\alpha}$ and $\cycle_{\bua\beta}$ at $\alpha$ and $\beta$,
respectively. At time $t_0^+$, both $\alpha$ and $\beta$ remain red. See
Figure~\ref{fig:transitions} (b).

Finally, consider the case when $(\ada, \alpha)$ is red and $(\adb, \alpha)$ is
blue. In this case, $\cycle_{\ada\alpha}^-$ contains $\cycle_{\adb\alpha}^-$ in
its interior. At time $t_0$, $\cycle_{\alpha=\beta}$ consists of three cycles
$\cycle_{\ada\alpha}, \cycle_{\adb\alpha}$, and $\cycle_{\bua\beta}$ ---
$\cycle_{\ada\alpha}$ containing both $\cycle_{\adb\alpha}$ and
$\cycle_{\bua\beta}$ in its interior with $\cycle_{\ada\alpha}$ touching
$\cycle_{\adb\alpha}$ at $\alpha$ and $\cycle_{\adb\alpha}$ touching
$\cycle_{\bua\beta}$ at $\beta$. At time $t_0^+$, $\alpha$ remains red but
$\beta$ becomes blue. See Figure~\ref{fig:transitions} (c).

We conclude this case by noticing that the case when $\alpha$ is blue can be
reduced to the third case above by reversing the direction of time.

\begin{figure}
\centering
\begin{tabular}{ |>{\centering\arraybackslash}m{.4cm}|| >{\centering\arraybackslash}m{2.0cm}| >{\centering\arraybackslash}m{3.1cm}| >{\centering\arraybackslash}m{3.1cm}| >{\centering\arraybackslash}m{3.1cm} | >{\centering\arraybackslash}m{2.0cm}| }
\hline
& $\contourtree$ & \multicolumn{3}{c|}{Contours} & $\contourtree$ \\
\cline{2-6}
& $t_0^-$ & $t_0^-$ & $t_0$ & $t_0^+$ & $t_0^+$ \\
\hline 
(a) & \includegraphics[width=0.10\textwidth, page=4]{figures/negative-interchange-transitiona} 
    & \includegraphics[width=0.20\textwidth, page=1]{figures/negative-interchange-transitiona} 
    & \includegraphics[width=0.20\textwidth, page=2]{figures/negative-interchange-transitiona}
    & \includegraphics[width=0.20\textwidth, page=3]{figures/negative-interchange-transitiona}
    & \includegraphics[width=0.10\textwidth, page=5]{figures/negative-interchange-transitiona} \\
\hline
(b) & \includegraphics[width=0.10\textwidth, page=4]{figures/negative-interchange-transitionb} 
    & \includegraphics[width=0.20\textwidth, page=1]{figures/negative-interchange-transitionb} 
    & \includegraphics[width=0.20\textwidth, page=2]{figures/negative-interchange-transitionb} 
    & \includegraphics[width=0.20\textwidth, page=3]{figures/negative-interchange-transitionb}
    & \includegraphics[width=0.10\textwidth, page=5]{figures/negative-interchange-transitionb} \\
\hline 
(c) & \includegraphics[width=0.10\textwidth, page=4]{figures/negative-interchange-transitionc} 
    & \includegraphics[width=0.20\textwidth, page=1]{figures/negative-interchange-transitionc} 
    & \includegraphics[width=0.20\textwidth, page=2]{figures/negative-interchange-transitionc}
    & \includegraphics[width=0.20\textwidth, page=3]{figures/negative-interchange-transitionc}
    & \includegraphics[width=0.10\textwidth, page=5]{figures/negative-interchange-transitionc} \\
\hline 

\end{tabular}
\caption{Illustration of topological changes in $\levelset$ and
  contour tree transitions during negative interchange events.  Dashed
  lines are contours at the height of $\alpha$ and solid lines are
  contours at the height of $\beta$. (a) is when $\cycle_{\beta}$ is
  blue. (b) and (c) are when $\cycle_{\beta}$ is red.}
\label{fig:transitions}
\end{figure}

\subsubsection{Mixed interchange event}
We now consider the case when $\alpha$ is negative and $\beta$ is positive. We
assume that the edge $(\alpha, \beta)$ is blue at $t_0^-$, so both $\alpha$ and
$\beta$ are blue at $t_0^-$. The case when $(\alpha, \beta)$ is red reduces to
this case by reversing the direction of the $z$-axis. Let $\ada$ and $\adb$ be
the two down neighbors of $\alpha$ and $\bua,\bub$ the up neighbors of $\beta$
at time $t_0^-$.  Both $(\ada,\alpha)$ and $(\adb,\alpha)$ are blue edges.
Assume that the edge $(\beta, \bua)$ is blue and $(\beta, \bub)$ is red.

Let $\cycle^-$ denote a contour at time $t_0^-$ for a point $\ext$ lying on the
(relative interior of the) edge ($\alpha, \beta)$, i.e. $\cycle^- =
\rho^{-1}(\ext)$.  Let $\cycle_{\alpha}^-, \cycle_{\beta}^-$ be the contours at
time $t_0^-$ passing through $\alpha$ and $\beta$ respectively.  Each of them
consists of two simple polygonal cycles as described in
Section~\ref{sec:neg-interchange}. The two cycles of $\cycle_{\alpha}^-$ lie in
the exterior of each other while one cycle of $\cycle_{\beta}^-$ lie in the
interior of the other. As $t_0^-$ approaches to $t_0$, $\cycle_{\alpha}^-$ and
$\cycle_{\beta}^-$ converge to each other, and let $\cycle_{\alpha=\beta}$ be
this contour at time $t_0$ --- passing through both $\alpha$ and $\beta$.

The vertices of $\cycle^-$ labeled with $\alpha$ form two connected components,
and the same is true for vertices labeled $\beta$. One of the up-contours
$\cycle_{\bub\beta}^-$ of $\cycle_\beta^-$ is red and the other up-contour
$\cycle_{\bua\alpha}^-$ of $\cycle_\beta^-$ is blue. All the edges in the edge
sequence $\seqedge(\cycle_{\bub\beta}^-)$ that are not incident to $\beta$
appear in $\seqedge(\cycle^-)$, and the same is true for
$\seqedge(\cycle_{\bua\beta}^-)$, as $\beta$ is the only vertex between them.
We mark the portion of $\cycle^-$ that intersects
$\seqedge(\cycle_{\bub\beta}^-)$ red and the portion that intersects
$\seqedge(\cycle_{\bua\beta}^-)$ blue. Note that red and blue portions of
$\cycle^-$ are delimited by the vertices that are labeled $\beta$. Similarly,
let $\cycle_{\ada\alpha}^-$ and $\cycle_{\adb\alpha}^-$ be the down-contours of
$\cycle_\alpha$, then all edges of $\seqedge(\cycle_{\ada\alpha}^-)$ and
$\seqedge(\cycle_{\adb\alpha}^-)$ that are not incident on $\alpha$ appear in
$\seqedge(\cycle^-)$. See Figure~\ref{fig:cycle_minus}

\begin{figure}
\centering
\begin{tabular}{ccc}
\includegraphics[width=0.3\textwidth,page=15]{figures/sign-interchange-proof.pdf} &
\includegraphics[width=0.3\textwidth,page=12]{figures/blue-proof.pdf} &
\includegraphics[width=0.3\textwidth,page=12]{figures/red-proof.pdf} \\
(a) & (b) & (c)
\end{tabular}
\caption{Possible forms of $\cycle^-$. Two saddles are depicted by $-$, $+$
saddles according to their sign. Hollow vertices has height higher the saddles
and filled vertices has height less than the saddles.} 
\label{fig:cycle_minus}
\end{figure}



There are three cases depending on the relative positions of the vertices
marked $\alpha$ and those marked $\beta$ in $\cycle^-$.
\\\\
(i) If the vertices marked $\alpha$ and those marked $\beta$ in $\cycle^-$ are
interleaved, then we refer to it as a \emph{sign-interchange} event.
\\\\
(ii) If the vertices marked $\alpha$ lie in the blue portion of $\cycle^-$,
then we refer to it as a \emph{blue} event.
\\\\
(iii) If the vertices marked $\alpha$ lie in the red portion of $\cycle^-$,
then we refer to it as a \emph{red} event.

In case (ii) and (iii), without loss of generality assume that the vertices
labeled $\beta$ intersect $\seqedge(\cycle_{\adb\alpha}^-)$.

The following lemma characterizes the change of $\contourtree$ at a mixed
interchange event.

\begin{lemma}
Assuming that the edge $(\alpha,\beta)$ is blue at $t_0^-$ and $\alpha$ lying
below $\beta$ at $t_0^-$, the following change occurs in $\contourtree$ at
$t_0$:
\\\\
(i) At a sign-interchange event, the topology of $\contourtree$ does not
change. The only change is that the label $\alpha$ and $\beta$ of
$\contourtree$ get swapped, so $\alpha$ becomes a positive (resp. negative)
saddle at $t_0^+$. See Figure~\ref{fig:mixed-transitions} (a).
\\\\
(ii) At a blue event, the signs of $\alpha$ and $\beta$ do not change, and the color of
$(\alpha, \beta)$ remains blue. At time $t_0^+$, $\adb$ is the down neighbor of
$\beta$, $\alpha$ and $\bub$ are the up neighbors of $\beta$, $\ada$ and
$\beta$ are down neighbors of $\alpha$, and $\bua$ is the up neighbor of
$\alpha$. See Figure~\ref{fig:mixed-transitions} (b).
\\\\
(iii) At a red event, the signs of $\alpha$ and $\beta$ do not change but the
edge $(\alpha, \beta)$ becomes red and so does the saddle $\alpha$; remains
$\beta$ a blue positive saddle. Furthermore, $\adb$ is down neighbor of
$\beta$, $\alpha$ and $\bua$ are the up neighbors of $\beta$, $\ada$ and
$\beta$ are down neighbors of $\alpha$, and $\bub$ is the up neighbor of
$\alpha$. See Figure~\ref{fig:mixed-transitions} (c).
\end{lemma}
\begin{proof}
We prove the case (i) in detail and sketch the proof for the other two cases,
as the argument is similar to case (i).

Consider the sign-interchange event. First we fix time $t_0^-$ and look at
contours in the neighborhood of $\alpha$ and $\beta$. Recall that $\cycle^-$ is
the contour at a point $\ext$ on the edge $(\alpha, \beta)$ of $\contourtree$.
As we walk from $\ext$ toward $\alpha$ on $(\alpha, \beta)$, $\cycle^-$
continuously deforms but its edge sequence does not change. As we reach the
node $\alpha$ of $\contourtree$, all vertices of $\cycle^-$ marked with
$\alpha$ converge to the vertex $\alpha$ of $\mesh$, and we obtain
$\cycle_\alpha^-$. Since the vertices marked $\alpha$ and $\beta$ in $\cycle^-$
are interleaved, each $\cycle_{\ada\alpha}^-$ and $\cycle_{\adb\alpha}^-$
contains the vertices marked $\beta$. Fix a height $\theta =
\heighttime{t_0^-}(\alpha) - \delta$ for some arbitrarily small $\delta > 0$.
Let $\cycle_\ada^-$ and $\cycle_\adb^-$ be the contours at height $\theta$
corresponding to edges $(\ada,\alpha)$ and $(\adb, \alpha)$, respectively, at
time $t_0^-$. Each of $\cycle_\ada^-$ and $\cycle_\adb^-$ also contains vertices
marked $\beta$ as well as vertices marked $\alpha$.

Next we fix the height $\theta$ and move forward in time to $t_0^+$. Let
$\cycle_\ada^+$ (resp. $\cycle_\adb^+$ be the contour at height $\theta$
corresponding to $\cycle_\ada^-$ (resp. $\cycle_\adb^-$). Since the only change
in $\heighttime{t_0^-}$ and $\heighttime{t_0^+}$ is that the height of $\alpha$
has crossed that of $\beta$, $\seqedge(\cycle_\ada^+) =
\seqedge(\cycle_\ada^-)$ and $\seqedge(\cycle_\adb^+) =
\seqedge(\cycle_\adb^-)$.

Now we fix the time to $t_0^+$ and increase the height from $\theta$ and
monitor how the contours $\cycle_\ada^+$ and $\cycle_\adb^+$ deform. Recall
that $\heighttime{t_0^+}(\beta) < \heighttime{t_0^+}(\alpha)$, so as we
increase the height, we first encounter $\beta$ and the vertices of
$\cycle_\ada^+, \cycle_\adb^+$ marked $\beta$ converge to the vertex $\beta$
of $\mesh$. Hence, $\beta$ is now a negative saddle. Since both $\cycle_\ada^+,
\cycle_\adb^+$ are blue, so is the saddle $\beta$ at $t_0^+$. The up-contour of
$\beta$ at time $t_0^+$ is a blue contour $\cycle^+$ such that
$\seqedge(\cycle^+)$ contains all edges of $\seqedge(\cycle_\ada^+) \cup
\seqedge(\cycle_\adb^+)$ that are not incident on $\beta$. If we continue to
increase the height, the vertices of $\cycle^+$ marked $\alpha$ converge to
$\alpha$ as we reach $\heighttime{t_0^+}(\alpha)$, and it splits into two contours at
$\alpha$. Since $\cycle^+$ was a blue contour, $\alpha$ is now a blue positive
saddle. $\contourtree$ still has the edge $(\beta,\alpha)$ corresponding to the
contours in the equivalence class of $\cycle^+$. This completes the proof of
the first part of the lemma.

Next if the vertices marked $\alpha$ and $\beta$ are not interleaved in
$\cycle^-$, then by our assumption the vertices marked $\beta$ lie in the cycle
$\cycle_{\adb\alpha}^-$ of $\cycle_\alpha^-$ and thus in the contour
$\cycle_\adb^-$ at height $\theta$; $\cycle_{\ada\alpha}^-$ and
$\cycle_{\ada}^-$ do not contain any vertex marked $\beta$. As we move the time
forward, the vertices marked $\beta$ lie in $\cycle_\adb^+$ and they are two
connected intervals in $\cycle_\adb^+$ that are marked $\beta$. Hence, as we
increase the height from $\theta$ to $\heighttime{t_0^+}(\beta)$ at time
$t_0^+$, the vertices marked $\beta$ in $\cycle_\adb^+$ converge to the vertex
$\beta$ of $\mesh$ and $\cycle_\adb^+$ splits into two contours at $\beta$.
Note that as we increase the height $\cycle_\ada^+$ also deforms but does not
meet $\beta$, as it has no vertices marked $\beta$. Hence $\beta$ is a blue
positive saddle, with $\adb$ as the down neighbor of $\beta$. Let
$\cycle_\beta^+$ be the contour passing through $\beta$ at time $t_0^+$. Let
$\cycle_{\bua\beta}^+, \cycle_{\bub\beta}^+$ be its two polygonal cycles.

If the blue event occurs, then $\cycle_{\bua\beta}^+$ contains the vertices
marked $\alpha$ so as we increase the height from $\heighttime{t_0^+}(\beta)$
to $\heighttime{t_0^+}(\alpha)$, the vertices marked $\alpha$ in
$\cycle_{\bua\beta}^+$ and $\cycle_{\ada}^+$ converge to $\alpha$, and the two
contours merge into a single contour $\cycle_\alpha^+$ at $\alpha$, implying
that $\alpha$ remains a negative saddle. Since the color of the up-contour
$\cycle_{\zeta\beta}^+$ is blue and $\cycle_{\ada}^+$ is also a blue contour, the
contour $\cycle_\alpha^+$ is blue, and thus $\alpha$ is a blue negative saddle.
The up-contour of $\cycle_\alpha^+$ is of the same equivalence class as
$\cycle_{\bua\beta}^-$. Hence, $\bua$ is the up neighbor of $\alpha$ in
$\contourtree$ at time $t_0^+$, and $\alpha$ and $\bub$ are the up neighbor of
$\beta$. This proves part (ii) of the lemma.

The proof for the third case is symmetric and omitted from here.
\end{proof}

The above lemma characterizes the changes in the contour tree at a mixed
interchange event under the assumption that $\alpha$ was a blue negative saddle
at $t_0^-$. As mentioned above, the other cases can be reduced to the above
case. In particular, if at time $t_0^-$, $\alpha$ is a red negative saddle,
reverse the direction of the $z$-axis; if $\alpha$ is a blue positive saddle,
reverse the direction of time; and if $\alpha$ is red positive saddle, then
reverse the direction of time as well as that of the $z$-axis.

\begin{figure}
\centering
\begin{tabular}{ |>{\centering\arraybackslash}m{.4cm}|| >{\centering\arraybackslash}m{2.0cm}| >{\centering\arraybackslash}m{3.1cm}| >{\centering\arraybackslash}m{3.1cm}| >{\centering\arraybackslash}m{3.1cm} | >{\centering\arraybackslash}m{2.0cm}| }
\hline
& $\contourtree$ & \multicolumn{3}{c|}{Contours} & $\contourtree$ \\
\cline{2-6}
& $t_0^-$ & $t_0^-$ & $t_0$ & $t_0^+$ & $t_0^+$ \\
\hline 
(a) & % \multirow{3}{*}{\includegraphics[width=0.10\textwidth, page=4]{figures/mixed-interchange-transitiona}}
    & \includegraphics[width=0.20\textwidth, page=1]{figures/mixed-interchange-transitiona} 
    & \includegraphics[width=0.20\textwidth, page=2]{figures/mixed-interchange-transitiona} 
    & \includegraphics[width=0.20\textwidth, page=3]{figures/mixed-interchange-transitiona} 
    & \includegraphics[width=0.10\textwidth, page=5]{figures/mixed-interchange-transitiona} \\
\cline{1-1} \cline{3-6} %\hline
(b) & \includegraphics[width=0.10\textwidth, page=4]{figures/mixed-interchange-transitionb} 
    & \includegraphics[width=0.20\textwidth, page=1]{figures/mixed-interchange-transitionb} 
    & \includegraphics[width=0.20\textwidth, page=2]{figures/mixed-interchange-transitionb} 
    & \includegraphics[width=0.20\textwidth, page=3]{figures/mixed-interchange-transitionb} 
    & \includegraphics[width=0.10\textwidth, page=5]{figures/mixed-interchange-transitionb} \\
\cline{1-1} \cline{3-6} %\hline %\hline 
(c) & % \includegraphics[width=0.10\textwidth, page=4]{figures/mixed-interchange-transitionc} 
    & \includegraphics[width=0.20\textwidth, page=1]{figures/mixed-interchange-transitionc} 
    & \includegraphics[width=0.20\textwidth, page=2]{figures/mixed-interchange-transitionc} 
    & \includegraphics[width=0.20\textwidth, page=3]{figures/mixed-interchange-transitionc} 
    & \includegraphics[width=0.10\textwidth, page=5]{figures/mixed-interchange-transitionc} \\
\hline 

\end{tabular}
\caption{Illustration of topological changes in $\levelset$ and
  contour tree transitions during mixed interchange events.  Dashed
  contour lines are contours at the height of $\alpha$ and solid
  contour lines are contours at the height of $\beta$. (a) Illustrates
  a sign change event. (b) Illustrates a blue event. (c) Illustrates a
  red event.}
\label{fig:mixed-transitions}
\end{figure}

\begin{figure} 
\centering
\begin{tabular}{|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{5cm}||>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{5cm}|}
\hline
\multicolumn{2}{|c||}{$t_0^-$} & \multicolumn{2}{c|}{$t_0^+$} \\
\hline
Height & Contours  & Height & Contours \\
\hline
$\heighttime{t_0^-}(\beta)+\delta$ &
\includegraphics[width=.3\textwidth, page=5]{figures/sign-interchange-proof} & 
$\heighttime{t_0^-}(\beta)+\delta$ &
\includegraphics[width=.3\textwidth, page=10]{figures/sign-interchange-proof} \\
\hline
$\heighttime{t_0^-}(\beta)$ $(\heighttime{t_0^+}(\beta))$ &
\includegraphics[width=.3\textwidth, page=6]{figures/sign-interchange-proof} & 
$\heighttime{t_0^+}(\alpha)$ &
\includegraphics[width=.3\textwidth, page=11]{figures/sign-interchange-proof} \\
\hline
$\heighttime{t_0^-}(\ext)$ $(\cycle^-)$&
\includegraphics[width=.3\textwidth, page=7]{figures/sign-interchange-proof} & 
$\heighttime{t_0^+}(\ext)$ $(\cycle^+)$&
\includegraphics[width=.3\textwidth, page=12]{figures/sign-interchange-proof} \\
\hline
$\heighttime{t_0^-}(\alpha)$ &
\includegraphics[width=.3\textwidth, page=8]{figures/sign-interchange-proof} & 
$\heighttime{t_0^+}(\beta)$ $(\heighttime{t_0^-}(\beta))$ &
\includegraphics[width=.3\textwidth, page=13]{figures/sign-interchange-proof} \\
\hline
$\heighttime{t_0^-}(\alpha)+\delta$ &
\includegraphics[width=.3\textwidth, page=9]{figures/sign-interchange-proof} & 
$\heighttime{t_0^-}(\alpha)+\delta$ &
\includegraphics[width=.3\textwidth, page=14]{figures/sign-interchange-proof} \\
\hline
\end{tabular}
\caption{Illustration of sign change event. The vertices marked $\alpha$ are
illustrated as red vertices and the vertices marked $\beta$ as blue vertices.
\jungwoo{Using $\ext$ at $t_0^+$ might be bad idea.}}
\label{fig:sign-interchange-proof}
\end{figure}

\begin{figure} 
\centering
\begin{tabular}{|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{5cm}||>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{5cm}|}
\hline
\multicolumn{2}{|c||}{$t_0^-$} & \multicolumn{2}{c|}{$t_0^+$} \\
\hline
Height & Contours  & Height & Contours \\
\hline
$\heighttime{t_0^-}(\beta)+\delta$ &
\includegraphics[width=.3\textwidth, page=10]{figures/blue-proof} & 
$\heighttime{t_0^-}(\beta)+\delta$ &
\includegraphics[width=.3\textwidth, page=11]{figures/blue-proof} \\
\hline
$\heighttime{t_0^-}(\beta)$ $(\heighttime{t_0^+}(\beta))$ &
\includegraphics[width=.3\textwidth, page=6]{figures/blue-proof} & 
$\heighttime{t_0^+}(\alpha)$ &
\includegraphics[width=.3\textwidth, page=9]{figures/blue-proof} \\
\hline
$\heighttime{t_0^-}(\ext)$ $(\cycle^-)$&
\includegraphics[width=.3\textwidth, page=5]{figures/blue-proof} & 
$\heighttime{t_0^+}(\ext)$ $(\cycle^+)$&
\includegraphics[width=.3\textwidth, page=8]{figures/blue-proof} \\
\hline
$\heighttime{t_0^-}(\alpha)$ &
\includegraphics[width=.3\textwidth, page=4]{figures/blue-proof} & 
$\heighttime{t_0^+}(\beta)$ $(\heighttime{t_0^-}(\beta))$ &
\includegraphics[width=.3\textwidth, page=7]{figures/blue-proof} \\
\hline
$\heighttime{t_0^-}(\alpha)+\delta$ &
\includegraphics[width=.3\textwidth, page=2]{figures/blue-proof} & 
$\heighttime{t_0^-}(\alpha)+\delta$ &
\includegraphics[width=.3\textwidth, page=3]{figures/blue-proof} \\
\hline
\end{tabular}
\caption{Illustration of blue event. The vertices marked $\alpha$ are
illustrated as red vertices and the vertices marked $\beta$ as blue vertices.
\jungwoo{Using $\ext$ at $t_0^+$ might be bad idea.}}
\label{fig:blue-proof}
\end{figure}

\begin{figure} 
\centering
\begin{tabular}{|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{5cm}||>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{5cm}|}
\hline
\multicolumn{2}{|c||}{$t_0^-$} & \multicolumn{2}{c|}{$t_0^+$} \\
\hline
Height & Contours  & Height & Contours \\
\hline
$\heighttime{t_0^-}(\beta)+\delta$ &
\includegraphics[width=.3\textwidth, page=10]{figures/red-proof} & 
$\heighttime{t_0^-}(\beta)+\delta$ &
\includegraphics[width=.3\textwidth, page=11]{figures/red-proof} \\
\hline
$\heighttime{t_0^-}(\beta)$ $(\heighttime{t_0^+}(\beta))$ &
\includegraphics[width=.3\textwidth, page=6]{figures/red-proof} & 
$\heighttime{t_0^+}(\alpha)$ &
\includegraphics[width=.3\textwidth, page=9]{figures/red-proof} \\
\hline
$\heighttime{t_0^-}(\ext)$ $(\cycle^-)$&
\includegraphics[width=.3\textwidth, page=5]{figures/red-proof} & 
$\heighttime{t_0^+}(\ext)$ $(\cycle^+)$&
\includegraphics[width=.3\textwidth, page=8]{figures/red-proof} \\
\hline
$\heighttime{t_0^-}(\alpha)$ &
\includegraphics[width=.3\textwidth, page=4]{figures/red-proof} & 
$\heighttime{t_0^+}(\beta)$ $(\heighttime{t_0^-}(\beta))$ &
\includegraphics[width=.3\textwidth, page=7]{figures/red-proof} \\
\hline
$\heighttime{t_0^-}(\alpha)+\delta$ &
\includegraphics[width=.3\textwidth, page=2]{figures/red-proof} & 
$\heighttime{t_0^-}(\alpha)+\delta$ &
\includegraphics[width=.3\textwidth, page=3]{figures/red-proof} \\
\hline
\end{tabular}
\caption{Illustration of red event. The vertices marked $\alpha$ are
illustrated as red vertices and the vertices marked $\beta$ as blue vertices.
\jungwoo{Using $\ext$ at $t_0^+$ might be bad idea.}}
\label{fig:blue-proof}
\end{figure}


